Uncover the Ground-Truth Relations in Distant Supervision: A Neural Expectation-Maximization Framework

Distant supervision for relation extraction enables one to effectively acquire structured relations out of very large text corpora with less human efforts. Nevertheless, most of the prior-art models for such tasks assume that the given text can be noisy, but their corresponding labels are clean. Such unrealistic assumption is contradictory with the fact that the given labels are often noisy as well, thus leading to significant performance degradation of those models on real-world data. To cope with this challenge, we propose a novel label-denoising framework that combines neural network with probabilistic modelling, which naturally takes into account the noisy labels during learning. We empirically demonstrate that our approach significantly improves the current art in uncovering the ground-truth relation labels.

==> assumption.tex <==
\begin{figure}[h]
	\centering 
	\includegraphics[width=\columnwidth]{CSCL.eps}
	\caption{clean sentence clean label}
	\label{fig:11}	
\end{figure}
\begin{figure}[h]
	\centering 
	\includegraphics[width=\columnwidth]{CSNL.eps}
	\caption{clean sentence noisy label}
	\label{fig:12}	
\end{figure}
\begin{figure}[h]
	\centering 
	\includegraphics[width=\columnwidth]{NSCL.eps}
	\caption{noisy sentence clean label}
	\label{fig:14}	
\end{figure}
\begin{figure}[h]
	\centering 
	\includegraphics[width=\columnwidth]{NSNL.eps}
	\caption{noisy sentence noisy label}
	\label{fig:15}	
\end{figure}

==> dataset.tex <==
\subsection{Datasets}
\subsubsection{The Riedel Dataset}
\label{sec:DS_data}
The Riedel dataset\footnote[2]{http://iesl.cs.umass.edu/riedel/ecml/} is a widely used DS dataset for relation extraction. It was developed in ~\cite{Riedel:10} through aligning entity pairs from Freebase with the New York Times (NYT) corpus.
%Entity mentions in the sentences are first recognized using the Stanford named entity recognizer~\cite{Finkel:05}. These mentions are then associated with entities in Freebase. For each associated entity pair $(e, e')$ in Freebase, all sentences in the corpus containing $e$ and $e'$ are collected to form a bag. Each relation between $(e, e')$ in Freebase is assigned as a label of the bag. When $e$ and $e'$ are not connected in Freebase, a special relation ``{\em NA}'' is assigned as the label. 
There are 53 relations in the Riedel dataset, including ``{\em NA}''. The bags collected from the 2005-2006 corpus are used as the training set, and the bags from the 2007 corpus are used as the test set. The training data contains $281,270$ entity pairs and $522,611$ sentences; the testing data contains $96,678$ entity pairs and $172,448$ sentences.

\subsubsection{TACRED Dataset}
TACRED is a large supervised relation extraction dataset collected in ~\cite{Zhang:17}. The text corpus is generated from the TAC KBP evaluation of years $2009-2015$. 
%The dataset contains 100 entities of people and organizations. Crowd workers are then asked to annotate the subject entity, object entity and the relation types of each sentence. 
Corpus from years $2009-2012$, year $2013$ and year $2014$ are used as training, validation and testing sets respectively. In all annotated sentences, $68,124$ are used for training, $22,631$ for validation and $15,509 $ for testing. There are $42$ relations in TACRED dataset, including a special relation ``{\em no relation}'', which is treated as NA in this study.
